Safety-Critical Kinematic Control of Robotic Systems

Over the decades, kinematic controllers have proven to be practically useful for applications like set-point and trajectory tracking in robotic systems. To this end, we formulate a novel safety-critical paradigm for kinematic control in this paper. In particular, we extend the methodology of control barrier functions (CBFs) to kinematic equations governing robotic systems. We demonstrate a purely kinematic implementation of a velocity-based CBF, and subsequently introduce a formulation that guarantees safety at the level of dynamics. This is achieved through a new form CBFs that incorporate kinetic energy with the classical forms, thereby minimizing model dependence and conservativeness. The approach is then extended to underactuated systems. This method and the purely kinematic implementation are demonstrated in simulation on two robotic platforms: a 6-DOF robotic manipulator, and a cart-pole system.

==> sections/double_integrator.tex <==

\section{Old/Extra Material}


\alert{Andrew: I originally wrote this section at a bit higher level, thinking I would introduce the theory later.  But since this is a control paper, want to do the theory first.  Thus I will rewrite a bit.  I put this here because you might want to use for the robotics journal.}

\subsection{Motivation}
\label{ssec:motivationint}

To motivate the kinematic control of robotic systems, consider the simplest example of a control system given by a (vector valued) single integrator: 
\begin{align}
\label{eqn:dotxu}
\dot{x} = v
\end{align}
for $x \in \R^n$ the state, assumed to be scalar, and $v \in \R^n$ also a scalar.  The first order nature of this system represents the kinematic nature of the control problem that will expanded upon later.  For this system, we wish to formulate safety-critical controller synthesis.  In this context, consider a safety function $h : \R^n \to \R$ defining a safe set: 
$$
\mathcal{S}  = \{ x \in \R^n ~ : ~ h(x) \geq 0\}.  
$$
That is, the system is ``safe'' when the function $h$ is positive.

% For example, $h(x) = x$ implies that the system should evolve in the set defined by $x \geq 0$, i.e., the positive real line. 

It is not possible to directly ensure safety of the system by simply checking on the positively of $h$.  Therefore, we can instead consider a derivative condition on $h$ that can be checked instantaneously.  Specifically, if $h$ is a \emph{control barrier function} \cite{ames2016control} if 
for all $x$ (in the domain of interest) there exists a $v$ such that:
%differentiating along solutions to \eqref{eqn:dotxu} yields: 
\begin{align}
\label{eqn:hdotsimple}
\dot{h}(x,u) = \frac{\partial h}{\partial x}(x) \dot{x} =
J_h(x) v \geq - \alpha h(x)
\end{align}
for $\alpha > 0$, where $J_h(x) = \frac{\partial h}{\partial x}(x) $ is the Jacobian of $h$.  In this case, given an input $v(x)$ that satisfies this inequality, consider the closed loop system $\dot{x} = v(x)$ with solution $x(t)$ and initial condition $x(0) = x_0$ wherein, because $v(x)$ satisfies \eqref{eqn:hdotsimple}: 
\begin{eqnarray}
\label{eqn:safetysimple}
x(0) = x_0 \in \mathcal{S} \qquad \Rightarrow \qquad 
x(t) \in \mathcal{S} \quad \forall ~ t \geq 0. 
\end{eqnarray}
Thus, the existence of a control barrier function implies safety. 

Control barrier functions can be used to synthesize controllers that ensure safety, as defined in \eqref{eqn:safetysimple}, even given a desired velocity: $v_{\rm des}(x,t)$.  
Specifically, the input $v \in \R^n$ can be explicitly found that satisfies the inequality in \eqref{eqn:hdotsimple} if $J_h(x) \neq 0$, i.e., if $h$ has \emph{relative degree} $1$ subject to minimizing the difference between this input and and the desired input.  This can be framed as an optimization problem, and specifically a quadratic program (QP): 
\begin{align}
\label{eqn:QPsimple}
v^*(x,t) = \underset{v \in \R^n}{\operatorname{argmin}} & ~  ~ \| v - v_{\rm des}(x,t) \|^2 \\
\mathrm{s.t.} & ~  ~ J_h(x) v \geq - \alpha h(x), \nonumber
\end{align}
where $v^*(x,t)$ is the pointwise optimal controller.  This controller has a closed form solution given by: 
\begin{align}
\label{eqn:minnormexplicitsimple}
& ~  v^*(x,t)  = \\
& \qquad 
\left\{ 
\begin{array}{lcr}
-J_h(x)^{\dagger}  \alpha h(x) & \mathrm{if~} J_h(x) v_{\rm des}(x,t) < - \alpha h(x) \\
v_{\rm des}(x,t) & \mathrm{if~} J_h(x) v_{\rm des}(x,t) \geq - \alpha h(x) 
\end{array}
\right.  \nonumber 
\end{align}
where 
$$
J_h(x)^{\dagger} = J_h(x)^{T}  (J_h(x) J_h(x)^T)^{-1} 
$$
is the Moore-Penrose (right) pseudoinverse.  
Therefore, this controller utilizes $v_{\rm des}$ whenever it is safe, i.e., when $J_h(x) v_{\rm des}(x,t) \geq - \alpha h(x)$.  Conversely, in the case when $v_{\rm des}$ is unsafe the controller takes over and enforces $\dot{h} = - \alpha h$ until $v_{\rm des}$ is safe again. 

It is interesting to consider the case when $v_{\rm des} = 0$, wherein the optimal controller in \eqref{eqn:QPsimple} becomes: 
\begin{align}
 v^*(x)  =
\left\{ 
\begin{array}{lcr}
-J_h(x)^{\dagger}  \alpha h(x)   & \mathrm{if~} h(x) < 0  \\
0 & \mathrm{if~} h(x) \geq 0
\end{array}
\right.   
\end{align}
Therefore, if the system starts in the safe set, $h(x) \geq 0$ and therefore $x \in \mathcal{S}$, the controller $v^*(x) = 0$ since for $\dot{x} = 0$ solutions will remain constant, and hence will stay in the set $\mathcal{S}$.  In the case when the system is outside of the safe set, i.e.,  $h(x) < 0$, the controller becomes $v^*(x) = -J_h(x)^{\dagger}  \alpha h(x)$ implying that $\dot{h}(x) = - \alpha h(x)$ which is just a stable linear system on the barrier function.  Thus $h(x(t)) = e^{-\alpha t}h(x(0)) \to 0$ exponentially.  To summarize, with this controller, the set $\mathcal{S}$ is safe and if the systems starts outside of this set it converges to it exponentially fast. 


\begin{example}[\textbf{Double integrator}]
Many robotic systems have second-order dynamics, but have distinct low-level and high-level controllers. The low-level controller operates at the forces and torques level, while the high-level controller gives velocity commands. It is often difficult to modify these low-level controllers, due to a lack of model information, or a lack of access to the torque control. In this case, the control barrier function must be implemented at the velocity level, and special consideration must be given to how the low-level controller can track these commands.

In the case of the double integrator, we have the system
\begin{align*}
    \dot{x} &= v \\
    \dot{v} &= u/m
\end{align*}

The low-level controller tracking velocities, in this example, is a simple P controller
\begin{align*}
    u &= mK(v-v_{\textrm{des}})
\end{align*}

When paired with the control barrier function given in \ref{eqn:QPsimple}, with the barrier $h(x) = 2^2-x^2$, we notice the dependence on the low-level controller gain $K$, illustrated in Figure \ref{fig:DI_K}. In the case of a lower gain, the system violates its barrier condition, and then returns to the boundary of the set. With the higher gain, however, the system stays safe. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/DI_K.png}
    \caption{Dependence on $K$}
    \label{fig:DI_K}
\end{figure}

This behavior is similar to the dependence that the barrier function has on the choice of $\alpha$, shown in Figure \ref{fig:DI_alpha} for a controller gain of $K = 2.5$.

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/DI_alpha.png}
    \caption{Dependence of $\alpha$}
    \label{fig:DI_alpha}
\end{figure}

It is clear that both the tracking performance of the low-level controller, as well as the scalar $\alpha$ in the CBF, affect the ability of these high-level CBFs to keep the underlying system invariant. This is, in part, due to the time-lag that exists between the safe velocity given by the barrier function, and the actual velocity of the system, as shown in Figure \ref{fig:time_lag}. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/time_lag.png}
    \caption{Velocity comparison}
    \label{fig:time_lag}
\end{figure}

\end{example}

==> sections/drone.tex <==


\begin{example}[\textbf{Connection with Potential Fields}]
Potential fields are employed for obstacle avoidance and goal attainment for single integrators.  In this context, one considers: 
\begin{itemize}
\item[\underline{\emph{Attractive:}}]  Given a goal state, $x_{\rm goal}$, one considers an \emph{attractive potential}, $U_{\rm att}$, which is a differentiable function with is ``quadratic'' in form, i.e., there exists $\underline{c}, \overline{c} > 0$ such that:
$$
\underline{c} \| x - x_{\rm goal} \|^2 \leq 
U_{\rm att}(x) \leq 
\overline{c} \| x - x_{\rm goal} \|^2. 
$$
\item[\underline{\emph{Repulsive:}}]  Given an obstacle at $x_{\rm obst}$ and minimum distance $D_{\rm obst} > 0$, one considers a \emph{repulsive potential}, $U_{\rm rep}$, that ``blows up'' at the minimum distance: 
$$
U_{\rm rep}(x) \geq 0  \quad \mathrm{and} \quad 
\lim_{\| x - x_{\rm obst}\| \to D_{\rm obst}} U_{\rm rep}(x) = \infty. 
$$
\end{itemize}
In the method of potential fields, combines thse attractive and repulsive forces into a single function: $U(x) = U_{\rm att}(x) + U_{\rm rep}(x)$ one then synthesizes a controller: 
$$
k(x) = - \nabla U(x)  \qquad \Rightarrow \qquad 
\dot{x} = - \nabla U(x), 
$$
where the gradient is just the Jacobian: $\nabla U(x) = J_U(x)$. 

The CBF paradigm includes potential fields as a special case.  To see this, we first note that from the repulsive potential we obtain a barrier function (this choice is not unique): 
$$
h_{\rm rep}(x) = \frac{1}{1 + U_{\rm rep}(x)} \quad \Rightarrow \quad 
J_{h_{\rm rep}}(x) = - \frac{1}{(1 + U_{\rm rep}(x))^2}. 
$$
Thus, because $U_{\rm rep}(x) \geq 0$ it implies that $J_{h_{\rm rep}}(x)$, $h$ is a valid relative 1 degree CBF.  Rather than combining the potentials as is done in the case of potential fields, we instead can realize the safety-critical controller via a QP: 
\begin{align}
\label{eqn:QPsimple}
v^*(x,t) = \underset{v \in \R^n}{\operatorname{argmin}} & ~  ~ \| v - 
\nabla U_{\rm att}(x) \|^2 \\
\mathrm{s.t.} & ~  ~  - \frac{v}{(1 + U_{\rm rep}(x))^2} \geq - \alpha(h(x)), \nonumber
\end{align}
This controller has an explicit solution as given in \eqref{eqn:minnormexplicitsimple}. 
\end{example}

\begin{example}[\textbf{Quadrotor}]
In this quadrotor example, we consider the case of a low-level attitude controller that is able to track desired velocity and yaw-rate commands.
\end{example}

==> sections/fullyact.tex <==

\subsection{Safety-Critical Control of Fully Actuated Robotic Systems}  

We begin by formulated a purely kinematic controller that guarantees that the dynamics stay within a subset of the safe set.  This will be achieved via a ``dynamically consistent'' extended CBF.  From this we can establish that a subset of the safe set is safe for the control system governing a robotic system through a controller that does not depend on these dynamics. 


\newsec{Dynamically consistent extended CBF.}  To dynamically extend the CBF, we note that the inertia matrix, $D(q)$ is a symmetric positive definite matrix, $D(q) = D(q)^T \succ 0$, and thus: 
$$
\lambda_{\min}(D(q)) \| q \|^2 \leq q^T D(q) q \leq
\lambda_{\max}(D(q)) \| q \|^2 
$$
where $\lambda_{\min}$ and $\lambda_{\max}$ are the maximum and minimum eigenvalues (which are dependent on $q$) of $D(q)$ which are necessarily positive due to the positive definite nature of $D(q)$.  Given a safety constraint expressed as a function $h : Q \subset \R^k \to \R$, i.e., a constraint that is only dependent on $q$, and the corresponding 0-superlevel set: $\S = \{ (q,\dot{q}) \in Q \times \R^k ~ : ~ h(q) \geq 0\}$.  Define the \emph{dynamically consistent extended CBF} as follows: 
\begin{eqnarray}
\label{eqn:dynCBF}
h_D(q, \dot{q}) := - \frac{1}{2} \dot{q}^T D(q) \dot{q} + h(q)
\end{eqnarray}
Note the similarity between this and the energy in a mechanical system, where the original function $h$ plays the role of the potential energy.  We can consider the safe set associated with this function: 
% $$
% \S_D = \{ (q,\dot{q} \in Q \times \R^k ~ : ~ h_D(q,\dot{q}) = 0 \} 
% $$
\begin{align}
\label{eqn:SD}
\S_D & : =   \{ (q,\dot{q} \in Q \times \R^k ~ : ~ h_D(q,\dot{q}) \geq 0 \}  \\
 & \subset  \{ (q,\dot{q} \in Q \times \R^k ~ : ~ h(q)  \geq \frac{1}{2} \lambda_{\min}(D(q)) \| \dot{q}  \|^2 \}  \subset \S  \nonumber
\end{align}
where the last inequality is implied by: $\frac{1}{2} \lambda_{\min}(D(q)) \| \dot{q}  \|^2 \geq 0$. 


\newsec{Control for dynamic safety.}  We can now establish the first main result of the paper.  That safety can be guaranteed for a robotic system via a controller that only depends on the kinematics and the gravity vector $G(q)$ and inertial matrix $D(q)$.  This makes the controller more robust to uncertainty in the dynamics then full model based controllers---which would require knowledge of the Coriolis matrix, $C(q,\dot{q})$, and is achieved using the dynamically extended CBF: $h_D$. 

% but comes at the cost of conservatism represented by the fact that $\S_D \subset \S$. 

% with associated control system \eqref{eqn:controlfromrobotic},

\begin{theorem} \label{thm:fully_actuated}
  Consider a robotic system \eqref{eqn:roboticsys}, assumed to be fully actuated with $B$ invertible, and a kinematic safety constraint $h : Q \to \R$ with corresponding safe set $\S = \{(q,\dot{q}) \in Q \times \R^k  :  h(q) \geq 0\}$.  Let $h_D$ be defined as in \eqref{eqn:dynCBF} with corresponding safe set $\S_D$ as given in \eqref{eqn:SD}. 
  Then $h_D$ is a control barrier function on $\S_D$ and given a desired controller $u_{\rm des}(x,t)$, the following controller for all $(q,\dot{q}) \in \S_D$:
% \begin{align}
% \label{eqn:QProbotic}
% u^*(q,\dot{q},t) = & ~ \underset{u \in \R^m}{\operatorname{argmin}}  ~  ~ \| u - u_{\rm des}(q,\dot{q},t) \|^2  \\
% ~ & \mathrm{s.t.}   ~ \underbrace{J_h(q)\dot{q}  - \dot{q}^T u + G(q)^T \dot{q}}_{\dot{h}_D(q,\dot{q},u)} \geq - \alpha(h_D(q,\dot{q})),  \nonumber
% \end{align}
\begin{gather}
\label{eqn:QProbotic}
\begin{split}
u^*(q,\dot{q},t) =  ~ \underset{u \in \R^m}{\operatorname{argmin}}  ~ & ~ \| u - u_{\rm des}(q,\dot{q},t) \|^2  \\
~  \mathrm{s.t.}   ~ & ~\underbrace{J_h(q)\dot{q}  - \dot{q}^T B u + G(q)^T \dot{q}}_{\dot{h}_D(q,\dot{q},u)} \geq - \alpha(h_D(q,\dot{q})),  
\end{split}
\end{gather}
guarantees forward invariance of $\S_D$, i.e., safety of $\S_D$.  Additionally, it has a closed form solution: 
\begin{gather}
\begin{split}
\label{eqn:minnormexplicitrobotic}
  u^*(x,t)  = u_{\rm des}(q,\dot{q},t) + 
%\qquad 
\left\{ 
\begin{array}{lcr}
\frac{B^T \dot{q}}{\|B^T  \dot{q} \|^2} \Psi(x,t;u_{\rm des})  & \mathrm{if~} \Psi(x,t; u_{\rm des}) < 0 \\
0 & \mathrm{if~} \Psi(x,t; u_{\rm des})  \geq 0
\end{array}
\right.   
\end{split}
\end{gather}
where 
\begin{gather}
\Psi(x,t;u_{\rm des}) := \dot{q}^T (J_h(q)^T  +  G(q) - B u_{\rm des}(x,t) ) + \alpha(h_D(q,\dot{q})) .  \nonumber
\end{gather}
%Finally, it renders $\S$ asymptotically stable.
\end{theorem}

\begin{remark}
It is important, and interesting to note that $h_D$ is a CBF on $\S_D$ without requiring that $h$ has relative degree 1, i.e., one need not require that $J_h(q) \neq 0$ as in Lemma \ref{lem:velocity}. 
\end{remark}

% \begin{remark}
% Note that this result is analogous to the fact that a PD controller together with gravity compensation: $u_{\rm PD}(q,\dot{q}) = G(q) - K_P (q - q_{\rm des}) - K_D \dot{q}$, which yields asympototic stability to the $(q_{\rm des},0)$.  In fact, this can be taken as the desired controller, $u_{\rm des} = u_{\rm PD}$, to yield stability subject to safety.  In this case, one need only know the potential energy of the system, not the complete dynamics. 
% % Importantly it is not necessarily to know the inertia matrix, $D(q)$, to ensure safety.  In particular, one need only pick initial conditions for the system of the form $(q,0) \in \S$ wherein $(q,0) \in \S_D$ since $h(q) = h_D(q,0)$.  The system \eqref{eqn:roboticsys}, under the controller \eqref{eqn:QProbotic}, will stay within $\S_D$ and hence $\S$. 
% \end{remark}


\begin{proof}
Note that the energy of the robotic system, $E(q,\dot{q}) = \frac{1}{2} \dot{q}^T D(q) \dot{q} + P(q)$ where $P(q)$ is the potential energy wherein the gravity vector $G(q) = \frac{\partial P}{\partial q}(q)$.  Differentiating $h_D$ along solutions yields (and suppressing the dependence on $q$ and $\dot{q}$): 
\begin{eqnarray}
\dot{h}_D  & = &   -\dot{q}^T D  \ddot{q} -\frac{1}{2} \dot{q}^T \dot{D} \dot{q} + J_h \dot{q} \nonumber\\
& = &  \dot{q}^T \left( C  \dot{q} + G  -  B u \right)  - \frac{1}{2} \dot{q}^T \dot{D} \dot{q} + J_h  \dot{q}  \nonumber\\
& = &  \frac{1}{2} \dot{q}^T \left( - \dot{D} + 2 C \right)\drew{\dot{q}}  - \dot{q}^T  B u  + G^T \dot{q} + J_h \dot{q} \nonumber\\
& =  &  - \dot{q}^T  B u  + G^T \dot{q} + J_h  \dot{q}  \nonumber
\end{eqnarray}
where the last %inequality
\drew{equality} follows from the fact that $\dot{D} - 2 C$ is skew symmetric.  

To establish that $h_D$ is a CBF, we need only show that \eqref{eqn:QProbotic} has a solution since the inequality constraint in \eqref{eqn:QProbotic} implies that \eqref{eqn:cbf:definition} is satisfied in Definition \ref{def:cbf}.
As a result of Lemma \ref{lem:explicitCBFsol}, the solution to \eqref{eqn:QProbotic} is given by \eqref{eqn:minnormexplicitrobotic}; this follows by noting: 
$$
L_f h_D(q,\dot{q})= (J_h(q) + G(q)^T ) \dot{q}, 
\qquad 
L_g h_D(q,\dot{q}) = \drew{-}\dot{q}^T B. 
$$
To show that \eqref{eqn:minnormexplicitrobotic} is well defined, we need to establish that: 
\begin{gather}
%L_f h_D(q,\dot{q}) = \dot{q}^T = 0  \qquad \Rightarrow \qquad L_g h_D (q,\dot{q}) + \alpha(h(q)) \geq 0. 
\drew{L_g h_D(q,\dot{q}) = -\dot{q}^T B = 0  \quad \Rightarrow \quad L_f h_D (q,\dot{q}) + \alpha(h_D(q,\dot{q})) \geq 0.} \nonumber
\end{gather}
Yet $\dot{q}^T B = 0$ implies that $\dot{q}^T= 0$ since $B$ is invertible and therefore
%$L_g h_D(q, \dot{q}) = 0$ 
\drew{$L_f h_D(q, \dot{q}) = 0$} and since $(q,\dot{q}) \in \S_D$ it follows that $h_D(q,\dot{q}) \geq 0$ and hence $\alpha(h_D(q,\dot{q})) \geq 0$ implying that \eqref{eqn:minnormexplicitrobotic} is well defined and thus $h_D$ is a CBF.  Finally, the results on the forward invariance of $\S_D$ follows from Theorem \ref{thm:cbf}. 

% To verify that $\S$ is forward invariant, by Nagumo's Theorem \cite{?} we need only establish that $\dot{h}(q,\dot{q}) = J_h(q) \dot{q} \geq 0$ for all $q$ such that $h(q) = 0$.  

% To verify that $\S_D$ is forward invariant, by Nagumo's Theorem \cite{?} we need only establish that $\dot{h}_D(q,\dot{q}) = \geq 0$ for all $(q,\dot{q})$ such that $h_D(q,\dot{q}) = 0$.  Yet this follows from the fact that:
% $$
% h_D(q,\dot{q}) = 0 \quad \Rightarrow \quad h(q) = \frac{1}{2} \dot{q}^T D(q) \dot{q} 
% \quad \Rightarrow \quad 
% $$
\end{proof}

% \textcolor{red}{The remark below is pretty obvious, but I think it's a nice property of the dynamically consistent CBF. It can make it pretty easy to pick an $h$ without being super confident in the model, and I've checked in sim that even if $\tilde{D} = 3D$, it's not as conservative as you would think.}
    

\begin{remark}
\drew{
If the $D$ is not known, or is uncertain, the safety guarantees from Theorem \ref{thm:fully_actuated} hold under the alternative constraint
\begin{equation}
    ~\underbrace{J_h(q)\dot{q}  - \dot{q}^T B u + G(q)^T \dot{q}}_{\dot{h}_D(q,\dot{q},u)} \geq - \alpha(\tilde{h}(q,\dot{q})),
\end{equation}
with $\tilde{h}(q,\dot{q}) \leq h_D(q,\dot{q})\ \forall (q,\dot{q}) \in \mathcal{S}_D$. For example, if $\tilde{h} = -\frac{1}{2} \dot{q}^T \tilde{D} \dot{q} + h$, and $\tilde{D}-D \succeq 0$, then $\tilde{h} \leq h_D$ and safety is guaranteed, since:
\begin{equation}
    ~\underbrace{J_h(q)\dot{q}  - \dot{q}^T B u + G(q)^T \dot{q}}_{\dot{h}_D(q,\dot{q},u)} \geq - \alpha(\tilde{h}(q,\dot{q})) \geq -\alpha(h_d(q,\dot{q})).
\end{equation}
An alternative condition is that $\lambda_{\min}(\tilde{D}) \geq \lambda_{\max}(D)$, which is easier to check but (potentially much) more conservative
    }
\end{remark}

% \newsec{Underactuated systems.}  We now consider the application of this methodology to underactuated systems, i.e., where $m < k$ and we have a non-trivial actuation matrix $B$.  Here, we can use the classical technique \cite{?} of converting the system to the ``task dynamics'' wherein, in the case of CBFs, this becomes the \emph{CBF dynamics}.  Applying the ``pre-feedback'' controller $u = B^T (J_h)^T u_h$, for $u_h \in \R$ the \emph{safety input}, and premultiplying by the transpose of the \emph{dynamically consistent} pseudoinverse: 


%\newsec{Underactuated systems.}  

\newsec{Connections with kinematic control.}  The goal is to now connect the previous constructions with the kinematic controllers defined in Section \ref{sec:kinematic}.   Concretely, often controllers can only be implemented as desired position and velocity commands that are passed to embedded level PD controllers.  As such, we consider a controller of the form: 
\begin{eqnarray}
\label{eqn:uDcont}
u = - K_{\rm vel}(\dot{q} - \dot{q}^*_d(q,\dot{q},t))
\end{eqnarray}
where $\dot{q}^*_d(q,t)$ is a desired velocity signal that enforces safety while trying to achieve tracking as in the case of Lemma \ref{lem:velocity} wherein we have a desired velocity based tracking controller: $\dot{q}_{\rm des}(q,t)  := J_y(q)^{\dagger} \left(\dot{x}_d(t) - \lambda (y(q) - x_d(t)) \right)$ for $\lambda > 0$.  The following is a result of the directly application of Theorem \ref{thm:fully_actuated} in the context of the controller \eqref{eqn:uDcont}. 

\begin{corollary}
Consider a robotic system \eqref{eqn:roboticsys}, and assume it is fully actuated.  Given a kinematic safety constraint $h : Q \to \R$ and the associated dynamically consistent extended CBF $h_D : Q \times \R \to \R$ as given in \eqref{eqn:dynCBF} with associated safe set $\S_D$, along with a desired trajectory $x_d(t)$ in the task space $x = y(q)$.  The D controller \eqref{eqn:uDcont} with $K_{\rm vel} \succ 0$ and:
\begin{gather}
\label{eqn:QProboticD}
\begin{split}
%q^*_d 
\dot{q}^*_d= ~
&  \underset{\dot{q}_d \in \R^n}{\operatorname{argmin}}  ~  ~ \| \dot{q}_d - \overbrace{J_y^{\dagger} \left(\dot{x}_d - \lambda (y - x_d) \right)}^{\dot{q}_{\rm des}(q,t)} \|^2  \\
&     \mathrm{s.t.}   ~  ~\underbrace{J_h \dot{q} +  \dot{q}^T B K_{\rm vel} \dot{q}  - \dot{q}^T B K_{\rm vel} \dot{q}_d + G^T \dot{q}}_{\dot{h}_D(q,\dot{q},\dot{q}_d)} \geq - \alpha(h_D),  
\end{split}
\end{gather}
guarantees forward invariance, i.e., safety, of $\S_D$.  Moreover, it has a closed form solution: 
\begin{gather}
\begin{split}
\label{eqn:minnormexplicitrobotic}
  %q^*_d
  \dot{q}^*_d= \dot{q}_{\rm des} + 
%\qquad 
\left\{ 
\begin{array}{lcr}
\frac{K_{\rm vel}^T B^T \dot{q}}{\|K_{\rm vel}^T B^T  \dot{q} \|^2} \Psi(q,\dot{q},t;q_{\rm des})  & \mathrm{if~} \Psi(q,\dot{q},t;q_{\rm des}) < 0 \\
0 & \mathrm{if~} \Psi(q,\dot{q},t;q_{\rm des}) \geq 0
\end{array}
\right.   
\end{split}
\end{gather}
where 
\begin{gather}
\Psi(q,\dot{q},t;%u_{\rm des})
\dot{q}_{\rm des}):= \dot{q}^T (J_h^T  +  G + 
%\dot{q}^T
B K_{\rm vel} \dot{q} - B K_{\rm vel} \dot{q}_{\rm des} ) + \alpha(h_D) .  \nonumber
\end{gather}
\end{corollary}
\drew{got rid of $\dot{q}$ in $\Psi$, changed $u_\text{des}$ and $q^*_d$ to $\dot{q}_{\rm des}$ and $\dot{q}^*_{\rm d}$}



==> sections/misc.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
\section{From Kinematics to Dynamics}
\label{sec:dynamics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now wish to establish the main result of this paper: that safety-critical kinematic control guarantees safety for the \emph{dynamics} of a robotic system. 

\newsec{Robotic Systems.}  We consider a robotic (or mechanical) system with configuration space $Q \subset \R^k$ with coordinates $q \in Q$ and equations of motion: 
\begin{eqnarray}
\label{eqn:roboticsys}
D(q) \ddot{q} + C(q,\dot{q}) \dot{q} + G(q) = B u
\end{eqnarray}
where $B \in \R^{k \times m}$ is the actuation matrix.  We assume $m \leq k$, wherein $m = k$ with $B = I$ corresponds to full actuation.
From the equations of motion, we can obtain a control system of the form \eqref{eqn:controlsys} (see \cite{?}).  

%From the equations of motion, we obtain a control system of the form \eqref{eqn:controlsys} with $x = (q, \dot{q}) \in \R^{2k}$ and:
% \begin{eqnarray}
% \label{eqn:controlfromrobotic}
%  \underbrace{\begin{bmatrix}
% \dot{q} \\
% \ddot{q} 
% \end{bmatrix}}_{\dot{x}}  = 
% \underbrace{\begin{bmatrix}
% \dot{q} \\
% -D(q)^{-1}\left( C(q,\dot{q}) \dot{q} +G(q) \right) 
% \end{bmatrix}}_{f(q,\dot{q})}
% + 
% \underbrace{\begin{bmatrix}
% 0 \\
% D(q)^{-1} B 
% \end{bmatrix}}_{g(q,\dot{q})} u.
% \end{eqnarray}

\subsection{Safety-Critical Control of Robotic Systems.}  

We begin by formulated a purely kinematic controller that guarantees that the dynamics stay within a subset of the safe set.  This will be achieved via a ``dynamically consistent'' extended CBF.  From this we can establish that a subset of the safe set is safe for the control system governing a robotic system through a controller that does not depend on these dynamics. 

\newsec{Dynamically consistent extended CBF.}  To dynamically extend the CBF, we note that the inertia matrix, $D(q)$ is a symmetric positive definite matrix and thus: 
$$
\lambda_{\min}(D(q)) \| q \|^2 \leq q^T D(q) q \leq
\lambda_{\max}(D(q)) \| q \|^2 
$$
where $\lambda_{\min}$ and $\lambda_{\max}$ are the maximum and minimum eigenvalues (which are dependent on $q$) of $D(q)$ which are necessarily positive due to the positive definite nature of $D(q)$.  Given a safety constraint expressed as a function $h : Q \subset \R^k \to \R$, i.e., a constraint that is only dependent on $q$, and the corresponding 0-superlevel set: $\S = \{ (q,\dot{q}) \in Q \times \R^k ~ : ~ h(q) \geq 0\}$.  Define the \emph{dynamically consistent extended CBF} as follows: 
\begin{eqnarray}
h_D(q, \dot{q}) := - \frac{1}{2} \dot{q}^T D(q) \dot{q} + h(q)
\end{eqnarray}
Note the similarity between this and the energy in a mechanical system, where the original function $h$ plays the role of the potential energy.  We can consider the safe set associated with this function: 
% $$
% \S_D = \{ (q,\dot{q} \in Q \times \R^k ~ : ~ h_D(q,\dot{q}) = 0 \} 
% $$
\begin{align}
\S_D & : =   \{ (q,\dot{q} \in Q \times \R^k ~ : ~ h_D(q,\dot{q}) \geq 0 \}  \nonumber\\
 & \subset  \{ (q,\dot{q} \in Q \times \R^k ~ : ~ h(q)  \geq \frac{1}{2} \lambda_{\min}(D(q)) \| \dot{q}  \|^2 \}  \subset \S  \nonumber
\end{align}
where the last inequality is implied by: $\frac{1}{2} \lambda_{\min}(D(q)) \| \dot{q}  \|^2 \geq 0$. 


\newsec{Kinematic control for dynamic safety.}  We can now establish the first main result of the paper.  That safety can be guaranteed for a robotic system via a controller that \emph{only} depends on the kinematics and the gravity vector $G(q)$.  This makes the controller robust to uncertainty in the dynamics, and is achieved using the dynamically extended CBF: $h_D$. 

% but comes at the cost of conservatism represented by the fact that $\S_D \subset \S$. 

% with associated control system \eqref{eqn:controlfromrobotic},

\begin{theorem}
  Consider a robotic system \eqref{eqn:roboticsys}, assumed to be fully actuated with $B = I$, and a safety constraint $h : Q \to \R$ with corresponding safe set $\S = \{(q,\dot{q}) \in Q \times \R^k  :  h(q) \geq 0\}$.  Given a desired controller $u_{\rm des}(x,t)$, then $h_D$ is a control barrier function on the set $\S_D$.  Moreover, the following controller for all $x \in \S_D$:
\begin{align}
\label{eqn:QProbotic}
u^*(x,t) = & ~ \underset{u \in \R^m}{\operatorname{argmin}}  ~  ~ \| u - u_{\rm des}(q,\dot{q},t) \|^2  \\
~ & \mathrm{s.t.}   ~ \underbrace{J_h(q)\dot{q} - \dot{q}^T u + G(q)^T \dot{q}}_{\dot{h}_D(q,\dot{q},u)} \geq - \alpha(h(q)),  \nonumber
\end{align}
guarantees forward invariance of $\S$, i.e., safety of $\S$.  Additionally, it renders $\S$ asymptotically stable.  Finally, it has a closed form solution: 
\begin{gather}
\begin{split}
\label{eqn:minnormexplicitrobotic}
  u^*(x,t)  = u_{\rm des}(q,\dot{q},t) + 
%\qquad 
\left\{ 
\begin{array}{lcr}
- \frac{\dot{q}}{\| \dot{q} \|^2} \Psi(x,t;u_{\rm des})  & \mathrm{if~} \Psi(x,t; u_{\rm des}) < 0 \\
0 & \mathrm{if~} \Psi(x,t; u_{\rm des})  \geq 0
\end{array}
\right.   
\end{split}
\end{gather}
where 
\begin{gather}
\Psi(x,t;u_{\rm des}) := \dot{q}^T (J_h(q)^T +  G(q) -  u_{\rm des}(x,t) ) + \alpha(h(x)) .  \nonumber
\end{gather}
\end{theorem}


\begin{remark}
Note that it is note necessarily to know the inertia matrix, $D(q)$, to ensure safety.  In particular, one need only pick initial conditions for the system of the form $(q,0) \in \S$ wherein $(q,0) \in \S_D$ since $h(q) = h_D(q,0)$.  The system \eqref{eqn:roboticsys}, under the controller \eqref{eqn:QProbotic}, will stay within $\S_D$ and hence $\S$. 
\end{remark}        

\begin{remark}
Note that this result is analogous to the fact that a PD controller together with gravity compensation: $u_{\rm PD}(q,\dot{q}) = G(q) - K_P (q - q_{\rm des}) - K_D \dot{q}$, which yields asympototic stability to the $(q_{\rm des},0)$.  In fact, this can be taken as the desired controller, $u_{\rm des} = u_{\rm PD}$, to yield stability subject to safety.  In this case, one need only know the potential energy of the system, not the complete dynamics.
\end{remark}


\begin{proof}
Note that the energy of the robotic system, $E(q,\dot{q}) = \frac{1}{2} \dot{q}^T D(q) \dot{q} + P(q)$ where $P(q)$ is the potential energy wherein the gravity vector $G(q) = \frac{\partial P}{\partial q}(q)$.  Differentiating $h_D$ along solutions yields (and suppressing the dependence on $q$ and $\dot{q}$): 
\begin{eqnarray}
\dot{h}_D  & = &   -\dot{q}^T D  \ddot{q} -\frac{1}{2} \dot{q}^T \dot{D} \dot{q} + J_h \dot{q} \nonumber\\
& = &  \dot{q}^T \left( C  \dot{q} + G  -  u \right)  - \frac{1}{2} \dot{q}^T \dot{D} \dot{q} + J_h  \dot{q}  \nonumber\\
& = &  \frac{1}{2} \dot{q}^T \left( - \dot{D} + 2 C \right)  - \dot{q}^T  u  + G^T \dot{q} + J_h \dot{q} \nonumber\\
& =  &  - \dot{q}^T  u  + G^T \dot{q} + J_h  \dot{q}  \nonumber
\end{eqnarray}
where the last inequality follows from the fact that $\dot{D} - 2 C$ is skew symmetric.  
Therefore, to establish that $h_D$ is a control barrier function on $\S_D$, assuming that $(q,\dot{q}) \in \S_D$, it implies that $h(q) \geq h_D(q,\dot{q}) \geq 0$ (since $\S_D \subset \S$).  Therefore: 
\begin{eqnarray}
u = G - J_h^T \quad &  \Rightarrow &  \quad 
\dot{h}_D = 0 \nonumber\\
\quad & \Rightarrow &  \quad  
\dot{h}_D  \geq - \alpha(h_D) \geq - \alpha(h) 
\nonumber
\end{eqnarray}
where the last inequalities follow from the fact that $-\alpha(h(q)) \leq - \alpha(h_D(q,\dot{q})) \leq 0$ since $\alpha$ is an extended class $\mathcal{K}$ function.  Thus, we have both established that $h_D$ is a CBF on $\S_D$ and the final inequality establishes that there exists a control input that satisfies the constraint in \eqref{eqn:QPacceleration}.

% where the last inequality follows from the fact that $\dot{D} - 2 C$ is skew symmetric.  Therefore, to establish that $h_e$ is a control barrier function on $\S_D$ we note that since we are assuming that $(q,\dot{q}) \in \S_D$ it implies that $h(q) \geq h_D(q,\dot{q}) \geq 0$.  Therefore: 
% \begin{eqnarray}
% u = G - J_h^T \quad \Rightarrow \quad 
% \dot{h}_D = 0 \quad \Rightarrow \quad  
% \begin{split}
%     \dot{h}_D & \geq - \alpha(h_D) \\
%      \dot{h}_D & \geq - \alpha(h) 
% \end{split}
% \nonumber
% \end{eqnarray}
% % \begin{eqnarray}
% % u = G - J_h^T \quad \Rightarrow \quad 
% % \dot{h}_D = 0 \quad \Rightarrow \quad  
% % \begin{split}
% %     \dot{h}_D & \geq - \alpha(h_D) \\
% %      \dot{h}_D & \geq - \alpha(h) 
% % \end{split}
% % \nonumber
% % \end{eqnarray}
% where the last inequalities follow from the fact that $-\alpha(h(q)) \leq - \alpha(h_D(q,\dot{q})) \leq 0$ since $\alpha$ is an extended class $\mathcal{K}$ function.  Thus, we have both established that $h_D$ is a CBF on $\S_D$ and the final inequality establishes that there exists a control input that satisfies the constraint in \eqref{eqn:QPacceleration}.

% \begin{eqnarray}
% u = G - J_h^T \quad \Rightarrow \quad 
% \dot{h}_D = 0 \quad \Rightarrow \quad  
% \begin{split}
%     \dot{h}_D & \geq - \alpha(h_D) \\
%      \dot{h}_D & \geq - \alpha(h) 
% \end{split}
% \nonumber
% \end{eqnarray}
% where the last inequalities follow from the fact that $-\alpha(h(q)) \leq - \alpha(h_D(q,\dot{q})) \leq 0$ since $\alpha$ is an extended class $\mathcal{K}$ function.  Thus, we have both established that $h_D$ is a CBF on $\S_D$ and the final inequality establishes that there exists a control input that satisfies the constraint in \eqref{eqn:QPacceleration}
\end{proof}




\newsec{Underactuated systems.}  We now consider the application of this methodology to underactuated systems, i.e., where $m < k$ and we have a non-trivial actuation matrix $B$.  Here, we can use the classical technique \cite{?} of converting the system to the ``task dynamics'' wherein, in the case of CBFs, this becomes the \emph{CBF dynamics}.  Applying the ``pre-feedback'' controller $u = B^T (J_h)^T u_h$, for $u_h \in \R$ the \emph{safety input}, and premultiplying by the transpose of the pseudoinverse $J_h^{\dagger} = J_h^T (J_h J_h^T)^{-1}$ of $J_h$, i.e., $J_h J_h^{\dagger} = I$ yields:
$$
(J_h^{\dagger})^T D \ddot{q} + 
(J_h^{\dagger})^T C(q,\dot{q}) \dot{q} + 
(J_h^{\dagger})^T  G(q) = 
(J_h^{\dagger})^T B B^T J_h^T u_h
$$
Now 
$$
D_h J_h = [J_h J_h^T]^{-1} J_h = 
\qquad 
(J_h^{\dagger})^T D = 
(J_h J_h^T)^{-1} J_h D 
$$




\subsection{Connections with Kinematic Control.}  

The goal is to now connect the previous constructions with the kinematic controllers defined in Section \ref{sec:kinematic}. 

\newsec{Velocity-based control.}
We begin by consider the controller $\dot{q}^*(q,t)$ obtained by solving \eqref{eqn:QPvelocity}.
% , which has explicit solution: 
% \begin{align}
% \label{eqn:minnormexplicitsimple2}
% & ~  \dot{q}^*(q,t)  = \\
% & \qquad 
% \left\{ 
% \begin{array}{lcr}
% -J_h(x)^{\dagger}  \alpha(h(x)) & \mathrm{if~} J_h(x) \dot{q}_{\rm des}(x,t) < - \alpha(h(x)) \\
% \dot{q}_{\rm des}(x,t) & \mathrm{if~} J_h(x) \dot{q}_{\rm des}(x,t) \geq - \alpha(h(x)) 
% \end{array}
% \right.  \nonumber 
% \end{align}
% where 
% $
% J_h(x)^{\dagger} = J_h(x)^{T}  (J_h(x) J_h(x)^T)^{-1} . 
% $
This desired value satisfies: 
$$
J_h(q) \dot{q}^*(q,t) \geq - \alpha(h(q)).
$$
We suppose this is implemented on the hardware as a simple D controller with gravity compensation: 
$$
u = k_{\rm vel}(q,t) = G(q) - K_{\rm vel}(\dot{q} - \dot{q}^*(q,t))
$$

%% NOTE: there was a sign error in this proof. 
% \begin{proof}
% Considering $h_D$ and calculating the derivative of this function with this controller applied yields (suppressing the dependence of functions on $q$ and $\dot{q}$): 
% \begin{eqnarray}
% \dot{h}_D & = & \dot{q}^T( -K_{\rm vel}(\dot{q} - \dot{q}^*(q,t)) + J_h^T ) \nonumber\\
% & = & -\dot{q}^T  K_{\rm vel} \dot{q}  + \dot{q}^T (J_h^T + \dot{q}^*(q,t)) \nonumber\\
% & \geq & -\lambda_{\max}( K_{\rm vel}) \| \dot{q} \|^2 + \dot{q}^T (J_h^T + \dot{q}^*(q,t)) \nonumber
% \end{eqnarray}
% Let $e(t) = \dot{q} - \dot{q}^*(q,t)$ and we assume that $\|e(t) \|_{\infty} = \limsup_{t \geq 0} \| e(t) \| $ be bounded, i.e., we have a velocity controller (perhaps at the embedded level) that achieves good tracking of the desired velocity $ \dot{q}^*(q,t)$.  Substituting this into the previous equation yields: 
% \begin{eqnarray}
% \dot{h}_D & \geq & -\lambda_{\max}( K_{\rm vel}) \| \dot{q} \|^2  \nonumber\\
% &&  + \dot{q}^*(q,t)^T  (J_h^T + \dot{q}^*(q,t)) + e^T  (J_h^T + \dot{q}^*(q,t)) \nonumber\\
% & \geq & -\lambda_{\max}( K_{\rm vel}) \| \dot{q} \|^2 - \alpha(h(q)) + \dot{q}^*(q,t)^T \dot{q}^*(q,t)  \nonumber\\
% && - \| e \|_{\infty} \| J_h^T \|  + (\dot{q} - \dot{q}^*(q,t))^T \dot{q}^*(q,t)   \nonumber\\
% & = & -\lambda_{\max}( K_{\rm vel}) \| \dot{q} \|^2  - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| + \dot{q}^T  \dot{q}^*(q,t) \nonumber\\
% & = & - \dot{q}^T \lambda_{\max}( K_{\rm vel})  (\dot{q} - \dot{q}^*(q,t)) - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| \nonumber\\
% & = & - \dot{q}^T \lambda_{\max}( K_{\rm vel})e - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| \nonumber\\
% & \geq & - \alpha(h(q))  
% - \|e\|_{\infty} \left( \lambda_{\max}(K_{\rm vel}) \|\dot{q} \| +  \| J_h^T \| \right) 
% \end{eqnarray}
% \end{proof}


\begin{proof}
Considering $h_D$ and calculating the derivative of this function with this controller applied yields (suppressing the dependence of functions on $q$ and $\dot{q}$): 
\begin{eqnarray}
\dot{h}_D  & = & \dot{q}^T (-G + K_{\rm vel}(\dot{q} - \dot{q}^*(q,t)) + G + J_h^T) \nonumber\\
& = & \dot{q}^T( K_{\rm vel}(\dot{q} - \dot{q}^*(q,t)) + J_h^T ) \nonumber\\
& = & \dot{q}^T  K_{\rm vel} \dot{q}  + \dot{q}^T (J_h^T - \dot{q}^*(q,t)) \nonumber\\
& \geq & \lambda_{\min}( K_{\rm vel}) \| \dot{q} \|^2 + \dot{q}^T (J_h^T - \dot{q}^*(q,t)) \nonumber\\
& \geq & \dot{q}^T (J_h^T - \dot{q}^*(q,t))
\end{eqnarray}
Let $e(t) = \dot{q} - \dot{q}^*(q,t)$ and we assume that $\|e(t) \|_{\infty} = \limsup_{t \geq 0} \| e(t) \| $ be bounded, i.e., we have a velocity controller (perhaps at the embedded level) that achieves good tracking of the desired velocity $ \dot{q}^*(q,t)$.  Substituting this into the previous equation yields: 
\begin{eqnarray}
\dot{h}_D & \geq &  \dot{q}^*(q,t)^T  (J_h^T - \dot{q}^*(q,t)) + e^T  (J_h^T - \dot{q}^*(q,t)) \nonumber\\
& \geq & - \alpha(h(q)) - \dot{q}^*(q,t)^T \dot{q}^*(q,t)  \nonumber\\
&& - \| e \|_{\infty} \| J_h^T \|  - (\dot{q} - \dot{q}^*(q,t))^T \dot{q}^*(q,t)   \nonumber\\
& = &  - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| - \dot{q}^T  \dot{q}^*(q,t)  \\
& = & 
 - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| - \dot{q}^T  (\dot{q} - e) \nonumber
\end{eqnarray}
\end{proof}






% \newsec{Velocity-based control.}
% We begin by consider the controller $\dot{q}^*(q,t)$ obtained by solving \eqref{eqn:QPvelocity}, which has explicit solution: 
% \begin{align}
% \label{eqn:minnormexplicitsimple2}
% & ~  \dot{q}^*(q,t)  = \\
% & \qquad 
% \left\{ 
% \begin{array}{lcr}
% -J_h(x)^{\dagger}  \alpha(h(x)) & \mathrm{if~} J_h(x) \dot{q}_{\rm des}(x,t) < - \alpha(h(x)) \\
% \dot{q}_{\rm des}(x,t) & \mathrm{if~} J_h(x) \dot{q}_{\rm des}(x,t) \geq - \alpha(h(x)) 
% \end{array}
% \right.  \nonumber 
% \end{align}
% where 
% $
% J_h(x)^{\dagger} = J_h(x)^{T}  (J_h(x) J_h(x)^T)^{-1} . 
% $
% This desired value satisfies: 
% $$
% J_h(q) \dot{q}^*(q,t) \geq - \alpha(h(q)).
% $$
% We suppose this is implemented on the hardware as a simple D controller with gravity compensation: 
% $$
% u = k_{\rm vel}(q,t) = G(q) + K_{\rm vel}(\dot{q} - \dot{q}^*(q,t))
% $$

% \begin{proof}
% Considering $h_D$ and calculating the derivative of this function with this controller applied yields (suppressing the dependence of functions on $q$ and $\dot{q}$): 
% \begin{eqnarray}
% \dot{h}_D & = & \dot{q}^T( K_{\rm vel}(\dot{q} - \dot{q}^*(q,t)) + J_h^T ) \nonumber\\
% & = & \dot{q}^T  K_{\rm vel} \dot{q}  + \dot{q}^T (J_h^T - \dot{q}^*(q,t)) \nonumber\\
% & \geq & \lambda_{\min}( K_{\rm vel}) \| \dot{q} \|^2 + \dot{q}^T (J_h^T - \dot{q}^*(q,t)) \nonumber\\
% & \geq & \dot{q}^T (J_h^T - \dot{q}^*(q,t))
% \end{eqnarray}
% Let $e(t) = \dot{q} - \dot{q}^*(q,t)$ and we assume that $\|e(t) \|_{\infty} = \limsup_{t \geq 0} \| e(t) \| $ be bounded, i.e., we have a velocity controller (perhaps at the embedded level) that achieves good tracking of the desired velocity $ \dot{q}^*(q,t)$.  Substituting this into the previous equation yields: 
% \begin{eqnarray}
% \dot{h}_D & \geq &  \dot{q}^*(q,t)^T  (J_h^T - \dot{q}^*(q,t)) + e^T  (J_h^T - \dot{q}^*(q,t)) \nonumber\\
% & \geq & - \alpha(h(q)) - \dot{q}^*(q,t)^T \dot{q}^*(q,t)  \nonumber\\
% && - \| e \|_{\infty} \| J_h^T \|  - (\dot{q} - \dot{q}^*(q,t))^T \dot{q}^*(q,t)   \nonumber\\
% & = &  - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| - \dot{q}^T  \dot{q}^*(q,t)  \\
% & = & 
%  - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| - \dot{q}^T  (\dot{q} - e) \nonumber
% \end{eqnarray}
% \end{proof}










% \begin{theorem}
%   Consider a robotic system \eqref{eqn:roboticsys}, assumed to be fully actuated with $B = I$, and a safety constraint $h : Q \to \R$ with corresponding safe set $\S = \{(q,\dot{q}) \in Q \times \R^k  :  h(q) \geq 0\}$.  Given a desired controller $u_{\rm des}(x,t)$, the following controller:
%   \begin{align}
% \label{eqn:QProbotic}
% u^*(x,t) = & ~ \underset{u \in \R^m}{\operatorname{argmin}}  ~  ~ \| u - u_{\rm des}(q,\dot{q},t) \|^2  \\
% ~ & ~ ~ \mathrm{s.t.}    \quad   \dot{q}^T G(q) - \dot{q}^T u  \geq - \alpha(h(q)) + \|J_h(q) \| \| \dot{q} \|,  \nonumber
% \end{align}
% guarantees safety of $\S$, i.e., forward invariance.  Additionally, it has a closed form solution: 
% \begin{gather}
% \begin{split}
% \label{eqn:minnormexplicitrobotic}
%   u^*(x,t)  = u_{\rm des}(q,\dot{q},t) + 
% %\qquad 
% \left\{ 
% \begin{array}{lcr}
% - \frac{\dot{q}}{\| \dot{q} \|^2} \Psi(x,t;u_{\rm des})  & \mathrm{if~} \Psi(x,t; u_{\rm des}) < 0 \\
% 0 & \mathrm{if~} \Psi(x,t; u_{\rm des})  \geq 0
% \end{array}
% \right.   
% \end{split}
% \end{gather}
% where 
% \begin{gather}
% \Psi(x,t;u_{\rm des}) := \dot{q}^T G(q) -   \dot{q}^T u_{\rm des}(x,t)  + \alpha(h(x)) -\|J_h(q) \| \| \dot{q} \| .  \nonumber
% \end{gather}
% Finally, this controller renders $\S$ asymptotically stable. 
% \end{theorem}

% \begin{gather}
% \begin{split}
% \label{eqn:minnormexplicitrobotic}
%   & u^*(x,t)  = u_{\rm des}(q,\dot{q},t) + 
% %\qquad 
% \left\{ 
% \begin{array}{lcr}
% - \frac{\dot{q}}{\| \dot{q} \|^2} \Psi(x,t;u_{\rm des})  & \mathrm{if~} \Psi(x,t; u_{\rm des}) < 0 \\
% 0 & \mathrm{if~} \Psi(x,t; u_{\rm des})  \geq 0
% \end{array} 
% \right.    \\
% & \qquad \Psi(x,t;u_{\rm des})  := \dot{q}^T G(q) -   \dot{q}^T u_{\rm des}(x,t)  + \alpha(h(x)) -\|J_h(q) \| \| \dot{q} \| . 
% \end{split} 
% \end{gather}


==> sections/misc2.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
\section{From Kinematics to Dynamics}
\label{sec:dynamics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now wish to establish the main result of this paper: that safety-critical kinematic control guarantees safety for the \emph{dynamics} of a robotic system. 

\newsec{Robotic Systems.}  We consider a robotic (or mechanical) system with configuration space $Q \subset \R^k$ with coordinates $q \in Q$ and equations of motion: 
\begin{eqnarray}
\label{eqn:roboticsys}
D(q) \ddot{q} + C(q,\dot{q}) \dot{q} + G(q) = B u
\end{eqnarray}
where $B \in \R^{k \times m}$ is the actuation matrix.  We assume $m \leq k$, wherein $m = k$ with $B = I$ corresponds to full actuation.
From the equations of motion, we can obtain a control system of the form \eqref{eqn:controlsys} (see \cite{?}).  

%From the equations of motion, we obtain a control system of the form \eqref{eqn:controlsys} with $x = (q, \dot{q}) \in \R^{2k}$ and:
% \begin{eqnarray}
% \label{eqn:controlfromrobotic}
%  \underbrace{\begin{bmatrix}
% \dot{q} \\
% \ddot{q} 
% \end{bmatrix}}_{\dot{x}}  = 
% \underbrace{\begin{bmatrix}
% \dot{q} \\
% -D(q)^{-1}\left( C(q,\dot{q}) \dot{q} +G(q) \right) 
% \end{bmatrix}}_{f(q,\dot{q})}
% + 
% \underbrace{\begin{bmatrix}
% 0 \\
% D(q)^{-1} B 
% \end{bmatrix}}_{g(q,\dot{q})} u.
% \end{eqnarray}

\subsection{Safety-Critical Control of Robotic Systems.}  

We begin by formulated a purely kinematic controller that guarantees that the dynamics stay within a subset of the safe set.  This will be achieved via a ``dynamically consistent'' extended CBF.  From this we can establish that a subset of the safe set is safe for the control system governing a robotic system through a controller that does not depend on these dynamics. 

\newsec{Dynamically consistent extended CBF.}  To dynamically extend the CBF, we note that the inertia matrix, $D(q)$ is a symmetric positive definite matrix and thus: 
$$
\lambda_{\min}(D(q)) \| q \|^2 \leq q^T D(q) q \leq
\lambda_{\max}(D(q)) \| q \|^2 
$$
where $\lambda_{\min}$ and $\lambda_{\max}$ are the maximum and minimum eigenvalues (which are dependent on $q$) of $D(q)$ which are necessarily positive due to the positive definite nature of $D(q)$.  Given a safety constraint expressed as a function $h : Q \subset \R^k \to \R$, i.e., a constraint that is only dependent on $q$, and the corresponding 0-superlevel set: $\S = \{ (q,\dot{q}) \in Q \times \R^k ~ : ~ h(q) \geq 0\}$.  Define the \emph{dynamically consistent extended CBF} as follows: 
\begin{eqnarray}
h_D(q, \dot{q}) := \frac{1}{2} \dot{q}^T D(q) \dot{q}
+
h(q)
\end{eqnarray}
% \begin{eqnarray}
% h_D(q, \dot{q}) := \underbrace{\frac{1}{2} \dot{q}^T D(q) \dot{q}}_{\textrm{kinetic energy}} 
% \hspace{0.8cm} + \hspace{-0.2cm}  
% \underbrace{h(q)}_{\textrm{ safety-critical 
% ``potential energy''}}
% \end{eqnarray}
Note the similarity between this and the energy in a mechanical system, where the original function $h$ plays the role of the potential energy.  Note that $h_D$ and $h$ are related via: 
\begin{eqnarray}
h_D(q,\dot{q}) \geq h(q) + \lambda_{\min}(D(q)) \| \dot{q} \|^2 \geq h(q)
\end{eqnarray}
Therfore, we can consider the safe set associated with $h_D$: 
\begin{align}
\S \subset \S_D  := \{ (q,\dot{q} \in Q \times \R^k ~ : ~ h_D(q,\dot{q}) \geq 0 \}  
\end{align}
Therefore, $\S \subset \S_D$.   It is important to note that these sets agree when $\dot{q} = 0$, i.e., if  $(q,0) \in \S$ then $(q,0) \in \S_D$ since $h(q) = h_D(q,0)$.  The deviation of these sets grows with $\| \dot{q} \|^2$.  



\newsec{Kinematic control for dynamic safety.}  We can now establish the first main result of the paper.  That safety can be guaranteed for a robotic system via a controller that \emph{only} depends on the kinematics and the gravity vector $G(q)$.  This makes the controller robust to uncertainty in the dynamics, and is achieved using the dynamically extended CBF: $h_D$. 

% but comes at the cost of conservatism represented by the fact that $\S_D \subset \S$. 

% with associated control system \eqref{eqn:controlfromrobotic},

\begin{theorem}
  Consider a robotic system \eqref{eqn:roboticsys}, assumed to be fully actuated with $B = I$, and a safety constraint $h : Q \to \R$ with corresponding safe set $\S = \{(q,\dot{q}) \in Q \times \R^k  :  h(q) \geq 0\}$.  Given a desired controller $u_{\rm des}(x,t)$, then $h_D$ is a control barrier function on the set $\S_D$.  Moreover, the following controller for all $x \in \S_D$:
\begin{align}
\label{eqn:QProbotic}
u^*(x,t) = & ~ \underset{u \in \R^m}{\operatorname{argmin}}  ~  ~ \| u - u_{\rm des}(q,\dot{q},t) \|^2  \\
~ & \mathrm{s.t.}   ~ \underbrace{J_h(q)\dot{q}  + \dot{q}^T u - G(q)^T \dot{q}}_{\dot{h}_D(q,\dot{q},u)} \geq - \alpha(h(q)),  \nonumber
\end{align}
guarantees forward invariance of $\S_D$, i.e., safety of $\S_D$.  Additionally, it has a closed form solution: 
\begin{gather}
\begin{split}
\label{eqn:minnormexplicitrobotic}
  u^*(x,t)  = u_{\rm des}(q,\dot{q},t) + 
%\qquad 
\left\{ 
\begin{array}{lcr}
- \frac{\dot{q}}{\| \dot{q} \|^2} \Psi(x,t;u_{\rm des})  & \mathrm{if~} \Psi(x,t; u_{\rm des}) < 0 \\
0 & \mathrm{if~} \Psi(x,t; u_{\rm des})  \geq 0
\end{array}
\right.   
\end{split}
\end{gather}
where 
\begin{gather}
\Psi(x,t;u_{\rm des}) := \dot{q}^T (J_h(q)^T -  G(q) + u_{\rm des}(x,t) ) + \alpha(h(q)) .  \nonumber
\end{gather}
Finally, it renders $\S_D$ asymptotically stable.
\end{theorem}

\begin{remark}
Note that it is note necessarily to know the inertia matrix, $D(q)$, to ensure safety with respect to $\S_D$ since, as noted above, $\S$ and $\S_D$ agree when $\dot{q} = 0$.  Additionally, while this result does not guarantee safety of $\S$, but rather the larger set $\S_D$, it does  

\end{remark}   

% \begin{remark}
% Note that it is note necessarily to know the inertia matrix, $D(q)$, to ensure safety.  In particular, one need only pick initial conditions for the system of the form $(q,0) \in \S$ wherein $(q,0) \in \S_D$ since $h(q) = h_D(q,0)$.  The system \eqref{eqn:roboticsys}, under the controller \eqref{eqn:QProbotic}, will stay within $\S_D$ and hence $\S$. 
% \end{remark}        


\begin{remark}
Note that this result is analogous to the fact that a PD controller together with gravity compensation: $u_{\rm PD}(q,\dot{q}) = G(q) - K_P (q - q_{\rm des}) - K_D \dot{q}$, which yields asympototic stability to the $(q_{\rm des},0)$.  In fact, this can be taken as the desired controller, $u_{\rm des} = u_{\rm PD}$, to yield stability subject to safety.  In this case, one need only know the potential energy of the system, not the complete dynamics.
\end{remark}


\begin{proof}
Note that the energy of the robotic system, $E(q,\dot{q}) = \frac{1}{2} \dot{q}^T D(q) \dot{q} + P(q)$ where $P(q)$ is the potential energy wherein the gravity vector $G(q) = \frac{\partial P}{\partial q}(q)$.  Differentiating $h_D$ along solutions yields (and suppressing the dependence on $q$ and $\dot{q}$): 
\begin{eqnarray}
\dot{h}_D  & = &   \dot{q}^T D  \ddot{q}  + \frac{1}{2} \dot{q}^T \dot{D} \dot{q} + J_h \dot{q} \nonumber\\
& = &  \dot{q}^T \left( - C  \dot{q} -  G  +  u \right)  + \frac{1}{2} \dot{q}^T \dot{D} \dot{q} + J_h  \dot{q}  \nonumber\\
& = &  \frac{1}{2} \dot{q}^T \left( \dot{D} - 2 C \right)  + \dot{q}^T  u  - G^T \dot{q} + J_h \dot{q} \nonumber\\
& =  &   \dot{q}^T  u  - G^T \dot{q} + J_h  \dot{q}  \nonumber
\end{eqnarray}
where the last inequality follows from the fact that $\dot{D} - 2 C$ is skew symmetric.  

To establish that $h_D$ is a CBF, we first prove that \eqref{eqn:QProbotic} is well defined.  The fact that the solution is given by \eqref{eqn:minnormexplicitrobotic} follows from Lemma \ref{lem:explicitCBFsol}, and the explicit solution given in that lemma, wherein one obtains \eqref{eqn:minnormexplicitrobotic} by noting that 
$$
L_f h_D(q,\dot{q})= J_h(q) - G(q)^T \dot{q}, 
\qquad 
L_g h_D(q,\dot{q}) = \dot{q}^T. 
$$
To show that \eqref{eqn:minnormexplicitrobotic} is well defined, i.e., that $h_D$ is a CBF per Definition \ref{def:cbf}, we need to establish that: 
$$
L_f h_D(q,\dot{q}) = \dot{q}^T = 0  \qquad \Rightarrow \qquad 
L_g h_D (q,\dot{q}) + \alpha(h(q)) \geq 0. 
$$
\end{proof}



==> sections/oldkincontrol.tex <==


\newsec{Velocity-based control.}
We begin by consider the controller $\dot{q}^*(q,t)$ obtained by solving \eqref{eqn:QPvelocity}.
% , which has explicit solution: 
% \begin{align}
% \label{eqn:minnormexplicitsimple2}
% & ~  \dot{q}^*(q,t)  = \\
% & \qquad 
% \left\{ 
% \begin{array}{lcr}
% -J_h(x)^{\dagger}  \alpha(h(x)) & \mathrm{if~} J_h(x) \dot{q}_{\rm des}(x,t) < - \alpha(h(x)) \\
% \dot{q}_{\rm des}(x,t) & \mathrm{if~} J_h(x) \dot{q}_{\rm des}(x,t) \geq - \alpha(h(x)) 
% \end{array}
% \right.  \nonumber 
% \end{align}
% where 
% $
% J_h(x)^{\dagger} = J_h(x)^{T}  (J_h(x) J_h(x)^T)^{-1} . 
% $
This desired value satisfies: 
$$
J_h(q) \dot{q}^*(q,t) \geq - \alpha(h(q)).
$$
We suppose this is implemented on the hardware as a simple D controller with gravity compensation: 
$$
u = k_{\rm vel}(q,\dot{q}, t) = G(q) - K_{\rm vel}(\dot{q} - \dot{q}^*(q,t))
$$

%% NOTE: there was a sign error in this proof. 
% \begin{proof}
% Considering $h_D$ and calculating the derivative of this function with this controller applied yields (suppressing the dependence of functions on $q$ and $\dot{q}$): 
% \begin{eqnarray}
% \dot{h}_D & = & \dot{q}^T( -K_{\rm vel}(\dot{q} - \dot{q}^*(q,t)) + J_h^T ) \nonumber\\
% & = & -\dot{q}^T  K_{\rm vel} \dot{q}  + \dot{q}^T (J_h^T + \dot{q}^*(q,t)) \nonumber\\
% & \geq & -\lambda_{\max}( K_{\rm vel}) \| \dot{q} \|^2 + \dot{q}^T (J_h^T + \dot{q}^*(q,t)) \nonumber
% \end{eqnarray}
% Let $e(t) = \dot{q} - \dot{q}^*(q,t)$ and we assume that $\|e(t) \|_{\infty} = \limsup_{t \geq 0} \| e(t) \| $ be bounded, i.e., we have a velocity controller (perhaps at the embedded level) that achieves good tracking of the desired velocity $ \dot{q}^*(q,t)$.  Substituting this into the previous equation yields: 
% \begin{eqnarray}
% \dot{h}_D & \geq & -\lambda_{\max}( K_{\rm vel}) \| \dot{q} \|^2  \nonumber\\
% &&  + \dot{q}^*(q,t)^T  (J_h^T + \dot{q}^*(q,t)) + e^T  (J_h^T + \dot{q}^*(q,t)) \nonumber\\
% & \geq & -\lambda_{\max}( K_{\rm vel}) \| \dot{q} \|^2 - \alpha(h(q)) + \dot{q}^*(q,t)^T \dot{q}^*(q,t)  \nonumber\\
% && - \| e \|_{\infty} \| J_h^T \|  + (\dot{q} - \dot{q}^*(q,t))^T \dot{q}^*(q,t)   \nonumber\\
% & = & -\lambda_{\max}( K_{\rm vel}) \| \dot{q} \|^2  - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| + \dot{q}^T  \dot{q}^*(q,t) \nonumber\\
% & = & - \dot{q}^T \lambda_{\max}( K_{\rm vel})  (\dot{q} - \dot{q}^*(q,t)) - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| \nonumber\\
% & = & - \dot{q}^T \lambda_{\max}( K_{\rm vel})e - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| \nonumber\\
% & \geq & - \alpha(h(q))  
% - \|e\|_{\infty} \left( \lambda_{\max}(K_{\rm vel}) \|\dot{q} \| +  \| J_h^T \| \right) 
% \end{eqnarray}
% \end{proof}


\begin{proof}
Considering $h_D$ and calculating the derivative of this function with this controller applied yields (suppressing the dependence of functions on $q$ and $\dot{q}$): 
\begin{eqnarray}
\dot{h}_D  & = & \dot{q}^T (-G + K_{\rm vel}(\dot{q} - \dot{q}^*(q,t)) + G + J_h^T) \nonumber\\
& = & \dot{q}^T( K_{\rm vel}(\dot{q} - \dot{q}^*(q,t)) + J_h^T ) \nonumber\\
& = & \dot{q}^T  K_{\rm vel} \dot{q}  + \dot{q}^T (J_h^T - \dot{q}^*(q,t)) \nonumber\\
& \geq & \lambda_{\min}( K_{\rm vel}) \| \dot{q} \|^2 + \dot{q}^T (J_h^T - \dot{q}^*(q,t)) \nonumber\\
& \geq & \dot{q}^T (J_h^T - \dot{q}^*(q,t))
\end{eqnarray}
Let $e(t) = \dot{q} - \dot{q}^*(q,t)$ and we assume that $\|e(t) \|_{\infty} = \limsup_{t \geq 0} \| e(t) \| $ be bounded, i.e., we have a velocity controller (perhaps at the embedded level) that achieves good tracking of the desired velocity $ \dot{q}^*(q,t)$.  Substituting this into the previous equation yields: 
\begin{eqnarray}
\dot{h}_D & \geq &  \dot{q}^*(q,t)^T  (J_h^T - \dot{q}^*(q,t)) + e^T  (J_h^T - \dot{q}^*(q,t)) \nonumber\\
& \geq & - \alpha(h(q)) - \dot{q}^*(q,t)^T \dot{q}^*(q,t)  \nonumber\\
&& - \| e \|_{\infty} \| J_h^T \|  - (\dot{q} - \dot{q}^*(q,t))^T \dot{q}^*(q,t)   \nonumber\\
& = &  - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| - \dot{q}^T  \dot{q}^*(q,t)  \\
& = & 
 - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| - \dot{q}^T  (\dot{q} - e) \nonumber
\end{eqnarray}
\end{proof}






% \newsec{Velocity-based control.}
% We begin by consider the controller $\dot{q}^*(q,t)$ obtained by solving \eqref{eqn:QPvelocity}, which has explicit solution: 
% \begin{align}
% \label{eqn:minnormexplicitsimple2}
% & ~  \dot{q}^*(q,t)  = \\
% & \qquad 
% \left\{ 
% \begin{array}{lcr}
% -J_h(x)^{\dagger}  \alpha(h(x)) & \mathrm{if~} J_h(x) \dot{q}_{\rm des}(x,t) < - \alpha(h(x)) \\
% \dot{q}_{\rm des}(x,t) & \mathrm{if~} J_h(x) \dot{q}_{\rm des}(x,t) \geq - \alpha(h(x)) 
% \end{array}
% \right.  \nonumber 
% \end{align}
% where 
% $
% J_h(x)^{\dagger} = J_h(x)^{T}  (J_h(x) J_h(x)^T)^{-1} . 
% $
% This desired value satisfies: 
% $$
% J_h(q) \dot{q}^*(q,t) \geq - \alpha(h(q)).
% $$
% We suppose this is implemented on the hardware as a simple D controller with gravity compensation: 
% $$
% u = k_{\rm vel}(q,t) = G(q) + K_{\rm vel}(\dot{q} - \dot{q}^*(q,t))
% $$

% \begin{proof}
% Considering $h_D$ and calculating the derivative of this function with this controller applied yields (suppressing the dependence of functions on $q$ and $\dot{q}$): 
% \begin{eqnarray}
% \dot{h}_D & = & \dot{q}^T( K_{\rm vel}(\dot{q} - \dot{q}^*(q,t)) + J_h^T ) \nonumber\\
% & = & \dot{q}^T  K_{\rm vel} \dot{q}  + \dot{q}^T (J_h^T - \dot{q}^*(q,t)) \nonumber\\
% & \geq & \lambda_{\min}( K_{\rm vel}) \| \dot{q} \|^2 + \dot{q}^T (J_h^T - \dot{q}^*(q,t)) \nonumber\\
% & \geq & \dot{q}^T (J_h^T - \dot{q}^*(q,t))
% \end{eqnarray}
% Let $e(t) = \dot{q} - \dot{q}^*(q,t)$ and we assume that $\|e(t) \|_{\infty} = \limsup_{t \geq 0} \| e(t) \| $ be bounded, i.e., we have a velocity controller (perhaps at the embedded level) that achieves good tracking of the desired velocity $ \dot{q}^*(q,t)$.  Substituting this into the previous equation yields: 
% \begin{eqnarray}
% \dot{h}_D & \geq &  \dot{q}^*(q,t)^T  (J_h^T - \dot{q}^*(q,t)) + e^T  (J_h^T - \dot{q}^*(q,t)) \nonumber\\
% & \geq & - \alpha(h(q)) - \dot{q}^*(q,t)^T \dot{q}^*(q,t)  \nonumber\\
% && - \| e \|_{\infty} \| J_h^T \|  - (\dot{q} - \dot{q}^*(q,t))^T \dot{q}^*(q,t)   \nonumber\\
% & = &  - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| - \dot{q}^T  \dot{q}^*(q,t)  \\
% & = & 
%  - \alpha(h(q)) - \| e \|_{\infty} \| J_h^T \| - \dot{q}^T  (\dot{q} - e) \nonumber
% \end{eqnarray}
% \end{proof}
